Privacy-Preserving Hierarchical Model-Distributed Inference

This paper focuses on designing a privacy-preserving Machine Learning (ML) inference protocol for a hierarchical setup, where clients own/generate data, model owners (cloud servers) have a pre-trained ML model, and edge servers perform ML inference on clients' data using the cloud server's ML model. Our goal is to speed up ML inference while providing privacy to both data and the ML model. Our approach (i) uses model-distributed inference (model parallelization) at the edge servers and (ii) reduces the amount of communication to/from the cloud server. Our privacy-preserving hierarchical model-distributed inference, privateMDI design uses additive secret sharing and linearly homomorphic encryption to handle linear calculations in the ML inference, and garbled circuit and a novel three-party oblivious transfer are used to handle non-linear functions. privateMDI consists of offline and online phases. We designed these phases in a way that most of the data exchange is done in the offline phase while the communication overhead of the online phase is reduced. In particular, there is no communication to/from the cloud server in the online phase, and the amount of communication between the client and edge servers is minimized. The experimental results demonstrate that privateMDI significantly reduces the ML inference time as compared to the baselines.

==> complexity_analysis.tex <==
\section{Discussion and Complexity Analysis} \label{sec:complexity analysis}

Table \ref{tab:framework_comparison} presents a comparison between Private MDI and other frameworks in terms of various features. The column "Layer Dist." indicates whether the framework distributes the layers across multiple parties. In this regard, SECO splits the ML model into two parts, while Private MDI is the only framework that leverages parallelization of the process. The "Collusion" column indicates whether the framework considers collusion among workers in their threat model. The "Nonlinearity" column evaluates the framework's ability to handle various nonlinear activation functions. For instance, SecureNN, Falcon, and SSNet employ specialized protocols for ReLU and Maxpooling, and they do not support other activation functions such as Tanh. This table highlights the unique capabilities of Private MDI in supporting parallelization and a wide range of nonlinear activation functions. 

The other columns in the table include "HE" (Homomorphic Encryption), "GC" (Garbled Circuits), and "SS" (Secret Sharing), which indicate the techniques used by each framework. The "Dataset" columns list the datasets used for evaluation, and the "ML Model" columns specify the machine learning models tested with each framework.


\begin{table*}[h!]
    \caption{Comparison of Private MDI with other frameworks. \fullcirc \hspace{0.25em} indicates the framework support a feature, \emptycirc \hspace{0.25em}indicates not supported feature, and \halfcirc \hspace{0.25em} refers the framework somehow supports the feature.}
    \label{tab:framework_comparison}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{>{\centering\arraybackslash}m{2cm} > {\centering\arraybackslash}m{1.5cm} >{\centering\arraybackslash}m{1.5cm} >{\centering\arraybackslash}m{1.5cm} >{\centering\arraybackslash}m{1.5cm} >{\centering\arraybackslash}m{1.5cm} >{\centering\arraybackslash}m{1.5cm} >
{\centering\arraybackslash}m{1.5cm} >{\centering\arraybackslash}m{1.5cm} >{\centering\arraybackslash}m{1.5cm} >{\centering\arraybackslash}m{1.5cm} >{\centering\arraybackslash}m{1.5cm} >{\centering\arraybackslash}m{1.5cm} >{\centering\arraybackslash}m{1.5cm} >{\centering\arraybackslash}m{1.5cm}}
\toprule
 
 \multirow{3}{*}{Framework} & \multirow{2}{*}{\rot{Layer Dist.}} & \multirow{2}{*}{\rot{Collusion}} & \multirow{2}{*}{\rot{Nonlinearity}} & HE & GC & SS & MNIST & CIFAR-10 & CIFAR-100 & Tiny ImageNet & MiniONN (MNIST) & MiniONN (CIFAR-10) & ResNet32 & VGG16 \\ 
 \cmidrule(lr){5-7} \cmidrule(lr){8-11} \cmidrule(lr){12-15}
 & & & & \multicolumn{3}{c}{Techniques} & \multicolumn{4}{c}{Dataset} & \multicolumn{4}{c}{ML Model} \\
 \cmidrule(lr){2-7} \cmidrule(lr){8-15}
 & \multicolumn{6}{c}{Theoretical Metrics} & \multicolumn{8}{c}{Evaluation Metrics} \\
\midrule
 SecureNN & \emptycirc & \emptycirc & \halfcirc & \emptycirc & \emptycirc & \fullcirc & \fullcirc & \emptycirc & \emptycirc & \emptycirc & \fullcirc & \emptycirc & \emptycirc & \emptycirc \\
 Falcon & \emptycirc & \emptycirc & \halfcirc & \emptycirc & \emptycirc & \fullcirc & \fullcirc & \fullcirc & \emptycirc & \fullcirc & \fullcirc & \emptycirc & \emptycirc & \fullcirc \\
 Delphi & \emptycirc & \emptycirc & \fullcirc & \fullcirc & \fullcirc & \fullcirc & \emptycirc & \fullcirc & \fullcirc & \emptycirc & \emptycirc & \fullcirc & \fullcirc & \emptycirc \\
 SECO & \halfcirc & \fullcirc & \fullcirc & \fullcirc & \fullcirc & \fullcirc & \fullcirc & \emptycirc & \fullcirc & \emptycirc & \fullcirc & \emptycirc & \fullcirc & \emptycirc \\
 SSNet & \emptycirc & \fullcirc & \halfcirc & \emptycirc & \emptycirc & \fullcirc & \fullcirc & \fullcirc & \emptycirc & \fullcirc & \emptycirc & \emptycirc & \halfcirc & \fullcirc \\
 Private MDI & \fullcirc & \halfcirc & \fullcirc & \fullcirc & \fullcirc & \fullcirc & \fullcirc & \fullcirc & \fullcirc & \fullcirc & \fullcirc & \fullcirc & \fullcirc & \fullcirc \\
\bottomrule
\end{tabular}}
\end{table*}


Table \ref{tab:comm_complexity} compares the number of rounds and communication complexity of Private MDI concerning Delphi and SecureNN. In this context, $T$ represents the number of colluding edge servers in a cluster, $N$ is the number of bits in a single input data $x \in \mathbb{Z}_q$, $\kappa$ denotes the length of the garbled circuit (GC) labels, $N_{enc}$ signifies the number of bits in homomorphically encrypted data, and $|GC|$ indicates the number of bits required to transmit the garbled circuits. Additionally, $h$ denotes the dimension of the square input matrix to a neural network (NN) layer, $g$ is the dimension of the kernel corresponding to the NN layer, and $i$ and $o$ represent the number of input and output channels, respectively. $p$ is the smaller field size in SecureNN \cite{securenn}.

Each row details the number of rounds and bits exchanged between the following pairs: the model owner and the data owner, the data owner and the edge server, and two edge servers. Notably, there is no communication between the model owner and edge servers. The critical insight from this table is that Private MDI aims to offload as much communication as possible to the edge servers and the offline phase. In contrast to Delphi, which follows a client-server model, Private MDI shifts the bottleneck (sending the GCs) to the edge servers and eliminates online phase communication between the client and the cloud server. SecureNN does not separate the protocol into online and offline phases. However, Private MDI emphasizes reducing online latency. By incorporating an offline phase, Private MDI halves the number of multiplications and minimizes the communication complexity for convolutional layers by a factor proportional to the kernel size. These optimizations lead to lower latency compared to Delphi and other approaches. In section \ref{sec:simulation results}, we validate our claims with simulation results.

Compared to the parallel work SECO \cite{chen2024seco}, their approach for the offline phase introduces additional homomorphic encryption computations for the second split of the ML model and increases the homomorphically encrypted communication overhead by a factor of three. Furthermore, during the online phase, the first part of the NN requires an interactive protocol with the client, similar to Delphi. Although SECO's code is not publicly available for direct comparison, our theoretical analysis indicates that Private MDI outperforms SECO in terms of offline phase latency and the removal of the client from the online phase.


\begin{table*}[h!]
    \caption{Comparison of communication complexities. MO: Model Owner, DO: Data Owner, and ES: Edge Server}
    \label{tab:comm_complexity}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{>{\centering\arraybackslash}m{1.5cm} > {\centering\arraybackslash}m{2cm} >{\centering\arraybackslash}m{0.5cm} >{\centering\arraybackslash}m{2cm} >{\centering\arraybackslash}m{0.5cm} >{\centering\arraybackslash}m{2cm} >
{\centering\arraybackslash}m{0.5cm} >{\centering\arraybackslash}m{2cm} >{\centering\arraybackslash}m{0.5cm} >{\centering\arraybackslash}m{2cm} >{\centering\arraybackslash}m{0.5cm} >{\centering\arraybackslash}m{2cm} >{\centering\arraybackslash}m{0.5cm} >{\centering\arraybackslash}m{2cm}}
\toprule
& \multirow{ 2}{*}{Layer Type} &\multicolumn{2}{c}{Delphi Offline}&\multicolumn{2}{c}{Delphi Online}&\multicolumn{2}{c}{SecureNN}&\multicolumn{2}{c}{Falcon}&\multicolumn{2}{c}{Private MDI Offline}&\multicolumn{2}{c}{Private MDI Online}\\ 
\cmidrule{3-14}
 & & Rds. & Comm. & Rds. & Comm. & Rds. & Comm. & Rds. & Comm. & Rds. & Comm. & Rds. & Comm. \\ 
\midrule
\multirow{2}{*}{MO-DO} & linear & 2 & $2N_{enc}$ & 2 & $2N$ & - & - & - & - & 2 & $2N_{enc}$ & - & - \\
& nonlinear & 3 & $|GC| + 2N\kappa$ & 1 & $N \kappa$ & - & - & - & - & - & - & - & - \\
\cmidrule{1-14}
\multirow{2}{*}{DO-ES} & linear & - & - & - & - & - & - & - & - & - & - & - & - \\ 
& nonlinear & - & - & - & - & - & - & - & - & 6 & $2N(2\kappa + 1)$ & - & - \\ 
\cmidrule{1-14}
\multirow{2}{*}{ES-ES} & linear & - & - & - & - & 2 & $(h^2g^2i + 2g^2oi + h^2o)N$ & $1$ & $(h^2o)N$ & - & - & 2 & $(h^2i + h^2o)N$ \\
& nonlinear & - & - & - & - & 10 & $(8\log p + 24)N$ & $5 + \log N$ & $0.5N$ & 1 & $|GC|$ & 1 & $N \kappa$ \\
\bottomrule
\end{tabular}}
\end{table*}


==> discussion.tex <==
\section{\label{sec:discuss}\pmdi in Perspective}
Table \ref{tab:framework_comparison} presents a comparison between Private MDI and other frameworks in terms of various features. The column "Layer Dist." indicates whether the framework distributes the layers across multiple parties. In this regard, SECO splits the ML model into two parts, while Private MDI is the only framework that leverages parallelization of the process. The "Collusion" column indicates whether the framework considers collusion among workers in their threat model. The "Nonlinearity" column evaluates the framework's ability to handle various nonlinear activation functions. For instance, SecureNN, Falcon, and SSNet employ specialized protocols for ReLU and Maxpooling, and they do not support other activation functions such as Tanh. This table highlights the unique capabilities of Private MDI in supporting parallelization and a wide range of nonlinear activation functions. 

The other columns in the table include "HE" (Homomorphic Encryption), "GC" (Garbled Circuits), and "SS" (Secret Sharing), which indicate the techniques used by each framework. The "Dataset" columns list the datasets used for evaluation, and the "ML Model" columns specify the machine learning models tested with each framework.


\begin{table*}[h!]
    \caption{Comparison of Private MDI with other frameworks. \fullcirc \hspace{0.25em} indicates the framework support a feature, \emptycirc \hspace{0.25em}indicates not supported feature, and \halfcirc \hspace{0.25em} refers the framework somehow supports the feature.}
    \label{tab:framework_comparison}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{>{\centering\arraybackslash}m{2cm} > {\centering\arraybackslash}m{1.5cm} >{\centering\arraybackslash}m{1.5cm} >{\centering\arraybackslash}m{1.5cm} >{\centering\arraybackslash}m{1.5cm} >{\centering\arraybackslash}m{1.5cm} >{\centering\arraybackslash}m{1.5cm} >
{\centering\arraybackslash}m{1.5cm} >{\centering\arraybackslash}m{1.5cm} >{\centering\arraybackslash}m{1.5cm} >{\centering\arraybackslash}m{1.5cm} >{\centering\arraybackslash}m{1.5cm} >{\centering\arraybackslash}m{1.5cm} >{\centering\arraybackslash}m{1.5cm} >{\centering\arraybackslash}m{1.5cm}}
\toprule
 
 \multirow{3}{*}{Framework} & \multirow{2}{*}{\rot{Layer Dist.}} & \multirow{2}{*}{\rot{Collusion}} & \multirow{2}{*}{\rot{Nonlinearity}} & HE & GC & SS & MNIST & CIFAR-10 & CIFAR-100 & Tiny ImageNet & MiniONN (MNIST) & MiniONN (CIFAR-10) & ResNet32 & VGG16 \\ 
 \cmidrule(lr){5-7} \cmidrule(lr){8-11} \cmidrule(lr){12-15}
 & & & & \multicolumn{3}{c}{Techniques} & \multicolumn{4}{c}{Dataset} & \multicolumn{4}{c}{ML Model} \\
 \cmidrule(lr){2-7} \cmidrule(lr){8-15}
 & \multicolumn{6}{c}{Theoretical Metrics} & \multicolumn{8}{c}{Evaluation Metrics} \\
\midrule
 SecureNN & \emptycirc & \emptycirc & \halfcirc & \emptycirc & \emptycirc & \fullcirc & \fullcirc & \emptycirc & \emptycirc & \emptycirc & \fullcirc & \emptycirc & \emptycirc & \emptycirc \\
 Falcon & \emptycirc & \emptycirc & \halfcirc & \emptycirc & \emptycirc & \fullcirc & \fullcirc & \fullcirc & \emptycirc & \fullcirc & \fullcirc & \emptycirc & \emptycirc & \fullcirc \\
 Delphi & \emptycirc & \emptycirc & \fullcirc & \fullcirc & \fullcirc & \fullcirc & \emptycirc & \fullcirc & \fullcirc & \emptycirc & \emptycirc & \fullcirc & \fullcirc & \emptycirc \\
 SECO & \halfcirc & \fullcirc & \fullcirc & \fullcirc & \fullcirc & \fullcirc & \fullcirc & \emptycirc & \fullcirc & \emptycirc & \fullcirc & \emptycirc & \fullcirc & \emptycirc \\
 SSNet & \emptycirc & \fullcirc & \halfcirc & \emptycirc & \emptycirc & \fullcirc & \fullcirc & \fullcirc & \emptycirc & \fullcirc & \emptycirc & \emptycirc & \halfcirc & \fullcirc \\
 Private MDI & \fullcirc & \halfcirc & \fullcirc & \fullcirc & \fullcirc & \fullcirc & \fullcirc & \fullcirc & \fullcirc & \fullcirc & \fullcirc & \fullcirc & \fullcirc & \fullcirc \\
\bottomrule
\end{tabular}}
\end{table*}


==> notation.tex <==
\section*{Appendix B: Notation Table} \label{notation}

Table \ref{tab:notation} provides a summary of the symbols used in the paper.

\begin{table*}[h!]
    \caption{Notation table.}
    \label{tab:notation}
    \centering
    \begin{tabular}{>{\centering\arraybackslash}m{2cm} >{\arraybackslash}m{15cm}}
        \toprule
        Symbol & Description \\
        \midrule
        $\mathbf{x}$ & Client's input. \\
        $\mathbf{x}_l$ & Output of the first $(l-1)$ layers of the ML model. \\
        $\mathbf{r}_l$ & Client's random sample. \\
        $\mathbf{s}_l$ & Cloud server's random sample. \\
        $\mathbf{c}_l$ & Function of client's random sample. \\
        $\mathbf{M}_l$ & ML model parameters corresponding to layer $l$. \\
        \texttt{(pk,sk)} & Pair of public key and secret key generated by the client for HE. \\
        $\mathbf{M}(\mathbf{x})$ & The inference result to input $\mathbf{x}$. \\
        $\mathbf{s}_l^{enc}$ & Homomorphically encrypted $\mathbf{s}_l$. \\
        $\mathbf{c}_l^{enc}$ & Homomorphically encrypted $\mathbf{c}_l$. \\
        $\mathbf{M}_l^{enc}$ & Homomorphically encrypted $\mathbf{M}_l$. \\
        $[\mathbf{s}_l]_v$ & Secret share of the cloud server's random sample sent to edge server $v$. \\
        $[\mathbf{M}_l]_v$ & Secret share of the ML model parameters corresponding to layer $l$ sent to edge server $v$. \\
        $C$ & The input circuit of the garbler server for the nonlinear activation function. \\
        $\Tilde{C}$ & The output garbled circuit of the garbler server. \\
        $\lambda$ & Security parameter of the GC. \\
        $L$ & Number of ML model layers. \\
        $P$ & Number of clusters. \\
        $\mathbb{Z}_q$ & Finite field of size $q$. \\
        $T$ & Maximum number of colluding edge servers in one cluster. \\
        $|GC|$ & Number of bits to send the garbled circuit and corresponding inner labels. \\
        $N$ & Number of bits of a single data $x \in \mathbb{Z}_q$. \\
        $N_{enc}$ & Number of bits of homomorphically encrypted data. \\
        $\kappa$ & Length of the labels of GC. \\
        \bottomrule
    \end{tabular}
\end{table*}
